NeurOCS: Neural NOCS Supervision for Monocular 3D Object Localization

Monocular 3D object localization in driving scenes is a crucial task, but challenging due to its ill-posed nature. Estimating 3D coordinates for each pixel on the object surface holds great potential as it provides dense 2D-3D geometric constraints for the underlying PnP problem. However, high-quality ground truth supervision is not available in driving scenes due to sparsity and various artifacts of Lidar data, as well as the practical infeasibility of collecting per-instance CAD models. In this work, we present NeurOCS, a framework that uses instance masks and 3D boxes as input to learn 3D object shapes by means of differentiable rendering, which further serves as supervision for learning dense object coordinates. Our approach rests on insights in learning a category-level shape prior directly from real driving scenes, while properly handling single-view ambiguities. Furthermore, we study and make critical design choices to learn object coordinates more effectively from an object-centric view. Altogether, our framework leads to new state-of-the-art in monocular 3D localization that ranks 1st on the KITTI-Object benchmark among published monocular methods.

==> sections/trash.tex <==
\noindent\textbf{Viewpoint Generalization.} 
Consider a slightly changed viewpoint $[\mathbf{R}', \mathbf{t}']$, where $\mathbf{p}_i$ corresponds to $\mathbf{p}_i' = \frac{\mathbf{R}' \hat{\mathbf{x}}_i + \mathbf{t}'}{ [\mathbf{R}' \hat{\mathbf{x}}_i + \mathbf{t}']_z} $ in the new viewpoint. 
For small viewpoint changes, a translation equivalent network (i.e. CNNs) tends to generalize through shifting the prediction $\tilde{\mathbf{x}}_i$ to $\mathbf{p}_i'$. In this case, the noise along the ray direction will be projected to the epipolar line of the new viewpoint and form a reprojection error as
\begin{equation} \label{eq:depth_noise_to_reproj_err}
    \frac{\mathbf{R}' \hat{\mathbf{x}}_i + \mathbf{t}' + \epsilon \mathbf{R}'\hat{\mathbf{R}}^T\mathbf{p}_i}{ [\mathbf{R}' \hat{\mathbf{x}}_i + \mathbf{t}' + \epsilon\mathbf{R}'\hat{\mathbf{R}}^T\mathbf{p}_i]_z} -
    \frac{\mathbf{R}'\hat{\mathbf{x}}_i + \mathbf{t}'}{ [\mathbf{R}'\hat{\mathbf{x}}_i + \mathbf{t}']_z}
    \approx\; \frac{ \epsilon\mathbf{R}'\hat{\mathbf{R}}^T\mathbf{p}_i }
    { [\mathbf{R}' \hat{\mathbf{x}}_i  + \mathbf{t}']_z}
\end{equation}
We made an approximation to simplify the equation under the assumption of  $[\epsilon\mathbf{R}'\hat{\mathbf{R}}^T\mathbf{p}_i]_z \!<\!\!<\! [\mathbf{R}'\hat{\mathbf{x}}_i + \mathbf{t}']_z$, where depth disturbance is relatively small compare to object depth under autonomous driving datasets.
Hence, the viewpoint change ($\mathbf{R}'\hat{\mathbf{R}}^T$) will project the shape corruption onto the reprojection error. 
This implies a generalization problem in testing time, that a particular viewpoint is not observed in the training data, but generalized from another viewpoint by shifting its coordinate prediction. The shape corruption will likely become a reprojection error that affects the PnP solver.
In practice, since the viewpoints are in continuous space, the effect ends up showing large errors for less observed viewpoints.
Our experiment [todo ref] consents with our theory that showing significantly degenerated performance under rare training viewpoints for the models trained with noisy shape supervisions.


\noindent\textbf{Geometric Consistency.} 
More generally, the shape corruption breaks the multi-view geometric consistency, where the reprojection error from viewpoint changing as in Eq.\eqref{eq:depth_noise_to_reproj_err} can be seen as a special case.
This limits the performance for utilizing the shape prediction for additional processes other than localization.
As an example, in experiment [todo], we fuse external dense depth estimations as scale priors by adding an extra term in PnP solver as
\begin{equation}
        \underset{\mathbf{R}, \mathbf{t}}{argmin} \sum_i \rho \Big(
    \frac{\mathbf{R} \mathbf{x}_i + \mathbf{t}}{[\mathbf{R} \mathbf{x}_i + \mathbf{t}]_z} - \mathbf{p}_i \Big) + \rho \Big( [\mathbf{R} \mathbf{x}_i + \mathbf{t}]_z - d_i \Big)
\end{equation}
With depth maps from stereo disparity estimation, a good shape supervision leads to competitive results to stereo methods, which doubled the precision of models trained with noisy shapes. 
Hence, a correct shape estimation that close to the real object shape can better couple with off-the-shelf geometric estimations, suggesting a better compatibility in a complex autonomous driving system that enforces geometry consistency from multiple sources (e.g. optical flow, multi-view stereo, lidar).




\noindent\textbf{NOC Branch.} 
For learning NOCs, we enforce the consistency between the network NOC prediction with the NOC rendering from Eq.\eqref{eq:render_noc}. For an image pixel $\mathbf{p}_i$ in normalized image coordinate, GT object pose $[\hat{\mathbf{R}}, \hat{\mathbf{t}}]$ and GT object size $\hat{\mathbf{s}}$, we obtain its corresponding viewing ray as 
\begin{equation}
    \mathbf{r}_i^{[\gamma]} = ( \gamma \hat{\mathbf{R}}^T\mathbf{p_i} - \hat{\mathbf{R}}^T\hat{\mathbf{t}} \big) ./ \hat{\mathbf{s}}
\end{equation}
where $./$ denotes the element-wise division.
We further predict a latent coefficient $\mathbf{z}$ for the object and obtain an object instance shape $\Phi_{obj}$ using Eq.\eqref{eq:phi_obj}. The NOC consistency loss is then written as
\begin{equation}
\begin{gathered}
   \mathcal{L}_{noc} = \frac{\sum_{i \in \Omega_{fg}} \alpha_i^{\star}(\mathbf{r}_i^{[\gamma_f]} \,|\, \Phi_{obj}) \cdot \big|\big|\, \mathbf{r}_{i}^{[noc]} \, \big|\big|^2} {\big|\Omega_{fg}\big|} 
   \\
   where \quad \mathbf{r}_{i}^{[noc]} =  \mathbf{o}_i - \mathbf{o}_i^{\star}(\mathbf{r}_i \,|\, \Phi_{obj}) 
\end{gathered}
\end{equation}
where $\Omega_{fg}$ denotes the foreground pixel set provided by the ground-truth mask.
Note although the predicted NOC is mainly a student who does not have provide shape information, we found enforcing this bi-directional consistency homogenize hard-to-learn high frequency details in the latent shape grid that speeds up the convergence. 




Additionally, we add a self supervised reprojection error loss~\cite{chen2021monorun}, which amplifies the loss orthogonal to the viewing ray direction as 
\begin{equation}
\begin{gathered}
   \mathcal{L}_{reproj} = \frac{\sum_{i \in \Omega_{fg}} \big|\big|\, \mathbf{r}_i^{[rep]} \, \big|\big|^2 } {\big|\Omega_{fg}\big|}
   \\
   where \quad \mathbf{r}_i^{[rep]} =  \frac{\hat{\mathbf{R}} (\hat{\mathbf{s}} \circ \mathbf{o}_i) + \hat{\mathbf{t}}} {[\hat{\mathbf{R}} (\hat{\mathbf{s}} \circ \mathbf{o}_i) + \hat{\mathbf{t}}]_z} - \mathbf{p}_i 
\end{gathered}
\end{equation}
Finally, we learn per-pixel foreground probability $w_{i}\!\in\![0,1]$ from ground-truth foreground mask, serve as weight in PnP problem as
\begin{equation}
    \mathcal{L}_{fg} = \frac{\sum_{i \in \Omega_{fg}} (1-w_i)^2} {\big|\Omega_{fg}\big|} + 
    \frac{\sum_{i \in \Omega_{fg}^c} (w_i)^2} {\big|\Omega_{fg}^c\big|}
\end{equation}
where $\Omega_{fg}^c$ is the complementary of $\Omega_{fg}$. 
We also implemented Aleatoric uncertainty same as \cite{chen2021monorun}, but found the different is only numerical. Hence, we simply kept the foreground probability as weight.




Finally, we learn per-pixel foreground probability $w_{i}\!\in\![0,1]$ from ground-truth foreground mask, serve as weight in PnP problem as
\begin{equation}
    \mathcal{L}_{fg} = \frac{\sum_{i \in \Omega_{fg}} (1-w_i)^2} {\big|\Omega_{fg}\big|} + 
    \frac{\sum_{i \in \Omega_{fg}^c} (w_i)^2} {\big|\Omega_{fg}^c\big|}
\end{equation}
where $\Omega_{fg}^c$ is the complementary of $\Omega_{fg}$. 
We also implemented Aleatoric uncertainty same as \cite{chen2021monorun}, but found the different is only numerical. Hence, we simply kept the foreground probability as weight.

==> supp_sections/additionaldetails.tex <==
\section{Supportive Explanations}

\noindent \textbf{NeRF grid configurations.} \label{sec:nerf_details}
Our NeRF representation rests on latent feature grids that can be efficiently decoded into color and density with a small MLP.
We use the implementation from \cite{tiny_cuda_nn} for latent grids that correspond to the space of a unit cubic. 
%We use a base width of 2 with 5 multi-scales and increase the width 2 times at each scale. This results in a maximum of grid resolution of $32 \!\times\! 32 \!\times\! 32$ at finest scale. 
In particular, we adopt the multi-resolution representation consisting of five latent grids, each with size $(2{\times}2{\times}2)$, $(4{\times}4{\times}4)$, $(8{\times}8{\times}8)$, $(16{\times}16{\times}16)$, and $(32{\times}32{\times}32)$. Each vertex on the grid stores a 4-dimensional learnable feature vector.
%Grid at each scale stores a 4-vector feature, 
Given a sampled point inside the 3D object box, we use its size-normalized NOCS to query each latent grid by trilinear interpolation, resulting in a total of $5{\times}4{=}20$ dimensional feature vector after concatenation. The feature vector is passed to an MLP containing three 64-channel hidden layers with ReLU activation, yielding color and density. We illustrate this procedure in \cref{fig:supp_gridnerf}, with two resolution scales for clarity of visualization. For each batch iteration during training, we randomly sample 768 rays per object to enforce rendering losses.

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth, trim = 0mm 38mm 60mm 0mm, clip]{figures/supp_gridnerf.pdf}
    \caption{\textbf{Illustration of our grid NeRF} that decodes color and density from a feature vector queried from latent grids. We use latent grids with five scales but only two are visualized for clarity.  }
    \label{fig:supp_gridnerf}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth, trim = 0mm 0mm 10mm 0mm, clip]{figures/supp_network.pdf}
    \caption{\textbf{Structure of our image-conditioned network} consisting of a backbone feature extraction network and a number of regression heads for different predictions.  
    }
    \label{fig:supp_network}
\end{figure}

\vspace{0.1cm}
\noindent \textbf{Base 3D detector.} It is worth stressing that the training of NeurOCS is agnostic to the base 3D detector -- NeurOCS takes ground truth 2D boxes as input in training, and during inference it is combined with a base 3D detector of choice, taking its 2D boxes as input. Also note the object size prediction is not needed during training. This makes  NeurOCS a standalone NOCS-based framework that can be flexibly combined with different base 3D detectors. In addition to DID-M3D, we show in next section that it also works well with another state-of-the-art 3D detector DEVIANT~\cite{kumar2022deviant}. As future work, we envision that NeurOCS has potential to improve Lidar-based 3D detection as well.

\vspace{0.1cm}
\noindent \textbf{Network architecture.} We illustrate our network pathways in \cref{fig:supp_network}. 
%We use ResNet50 pretrained on ImageNet as backbone. 
We crop objects using 2D boxes and resize to $256\!\times\!256$ as input to our backbone network, a ResNet50 pretrained on ImageNet. We extract its  $8{\times}8$ feature map at the fourth layer, upsample to $64{\times}64$ by bilinear interpolation, and then pass to a few regression heads. We apply three separate heads to predict the NOCS map, the uncertainty map (detailed later), and the foreground object mask, each using three $1{\times}1$ convolutional layers with BachNorm and ReLu activation.
The shape and color coefficients are predicted by a 3-layer MLP with the average-pooled feature map as input. The score prediction head uses two $1\!\times\!1$ convolutional layers followed by average-pooling and a linear layer to regress a confidence score. It takes as input the object feature map, the predicted NOCS map, the predicted foregound object mask, and the Jacobian map.
 



\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth, trim = 0mm 80mm 0mm 0mm, clip]{figures/supp_objmask.pdf}
    \caption{\textbf{Illustration of our ground-truth object mask.} The white, black, and gray pixels indicate foreground, background, and unknown regions, respectively.}
    \label{fig:supp_objectmask}
\end{figure}

\vspace{0.1cm}
\noindent \textbf{Foreground object masks.} We demonstrate our ground-truth object mask with two example objects in \cref{fig:supp_objectmask}. The foreground and background regions provide shape constraints in our occupancy loss akin to the machinery of shape-from-silhouette. Pixels on other object instances are ignored as they are likely occluding objects that obscure the shape boundary.


\begin{table}
    \centering
    \renewcommand{\arraystretch}{1.1}
    \resizebox{0.9\columnwidth}{!}{%
        \input{tables/supp_losses}
    }
    \caption{\textbf{A summary of our losses}, including NeRF losses and image-conditioned regression losses. See text for details.  }
    \label{table:losses}
\end{table}

\vspace{0.1cm}
\noindent \textbf{Shape Regularization}. We demonstrate the impact of the KL divergence loss in \cref{fig:visual_hull_ambiguity}(a), illustrate the visual hull ambiguity and that the dense prior improves the shape \cref{fig:visual_hull_ambiguity}(b).

\vspace{0.1cm}
\noindent \textbf{Loss.} We jointly train the image-conditioned regression network and the NeRF by combining all their losses. In \cref{table:losses}, we detail the training losses composition, including their weight, application scope and  condition. 
%The occupancy, FG, RGB and reprojection losses are normalized to $[0,1]$ (w/o square). 
%The NOCS consistency, Lidar, LiComp losses computes the difference between NOCS, hence range in $[0,2]$ (w/o square). 
The occupancy loss is applied on foreground and background, while skipping unknown regions. The RGB loss is only applied to the foreground region. If a point from Lidar or its completion resides inside the object 3D box and projects to the foreground region, it induces a valid NOCS point for supervision. The dense prior loss is applied to randomly sampled points inside the 3D latent grid; and it is  only applied in absence of Lidar/LiComp losses, hence marked as conditional. 
The NOCS consistency loss is applied to foreground regions and weighted by a detached occupancy map rendered from NeRF. 
We also add an unsupervised reprojection loss~\cite{chen2021monorun}, and similarly to~\cite{chen2021monorun} we learn a per-pixel aletoric uncertainty map $(\sigma_x,\sigma_y)$ for the NOCS projection on image in both horizontal and vertical diction, by optimizing $\frac{|\Delta p_x|^2}{\sigma_x^2}+\log\sigma_x^2$, where $|\Delta p_x|^2$ indicates the reprojection error in $x$ direction; same applies to $\sigma_y$. The confidence $(\frac{1}{\sigma_x},\frac{1}{\sigma_y})$ is multiplied with the foreground probability to weigh each pixel in PnP optimization, which also optimizes the reprojection error loss.
The weights combining the losses are chosen empirically based on the validation set, and we note that the performance is not sensitive to these parameters in practice.


\noindent \textbf{Data augmentation.} During the training, we apply data augmentation on the ground truth 2D boxes, including flipping and bounding box perturbation similar to~ \cite{li2019cdpn}.


\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/visual_hull.pdf}
    \caption{\textbf{Shape Regularizations.} (a) An actual example showing the KL loss yields cleaner shape. (b) An illustration on the visual hull ambiguity and the impact of the dense shape prior.
    }
    \label{fig:visual_hull_ambiguity}    
\end{figure}

==> supp_sections/additionalexp.tex <==
\section{Additional Experimental Results}


\subsection{Additional Results on KITTI}


\begin{table}
    \centering
    \renewcommand{\arraystretch}{1.1}
    \resizebox{1.0\columnwidth}{!}{%
        \input{tables/supp_comparewith_deviant}
    }
    \caption{Evaluation with DEVIANT~\cite{kumar2022deviant} as our base 3D detector.}
    \label{table:comparewith_deviant}
\end{table}



\begin{table}
    \centering
    \renewcommand{\arraystretch}{1.1}
    \resizebox{1.0\columnwidth}{!}{%
        \input{tables/supp_comparewith_cmkd}
    }
    \caption{Additional comparison with LPCG~\cite{peng2022lidar} and CMKD~\cite{hong2022cross} on KITTI test set. }
    \label{table:comparewith_cmkd}
\end{table}


\noindent \textbf{Base 3D detector.} We demonstrated good performance with DID-M3D~\cite{peng2022did} as our base 3D detector in the main paper. Here, we evaluate performance by combining NeurOCS with another base 3D detector, namely DEVIANT~\cite{kumar2022deviant}. As can be seen in \cref{table:comparewith_deviant}, NeurOCS improves over DEVIANT with the scale fusion, whether the shape is trained with mask only or with additional Lidar supervision. This further consolidates the value of NeurOCS as a standalone shape-based 3D localization framework. 

\if false
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/bidir.pdf}
    \caption{Three object instances demonstrating that the bi-directional NOCS consistency yields slightly smoother and better shapes.}
    \label{fig:bidir}
\end{figure}
\fi










\noindent \textbf{Additional comparison on KITTI benchmark.} In the main paper, we primarily compare with existing methods that rely on the original 3D box annotations from KITTI to train the 3D detector. However, it is also worth discussing recent works LPCG~\cite{peng2022lidar} and CMKD~\cite{hong2022cross} that improve performance by leveraging additional pseudo ground truth from extra large-scale unlabeled sequences with Lidar. %The pseudo ground truth is given by Lidar-based inference which further constrains the outputs from image-based networks during training.
While this line of work is orthogonal to ours, we provide performance comparison in \cref{table:comparewith_cmkd}. As shown, the accuracy from NeurOCS is superior to LPCG and comparable to CMKD.
%NeurOCS outperforms CMKD if they are trained with the original annotations, while CMKD achieves slightly better results if using the additional Lidar-based pseudo ground truth. It is important to note that our key contributions in NeurOCS are orthogonal to the advancements in the base 3D detector, \eg by leveraging unlabeled data as in CMKD, and both of them contribute to the final improvement in 3D localization, as we have shown.

\noindent \textbf{w/o NeRF results.} In the main paper, we have compared the PnP results from our NeRF-based method against directly training with raw depth supervision from Lidar and its completion w/o NeRF. Here, we report in \cref{table:withoutnerf} the full $AP_{3D}$ for the ``w/o NeRF" setting including the results after scale fusion. Note that we always include the reprojection error loss as it was shown helpful~\cite{chen2021monorun} for NOCS learning. As can be seen, the direct training yields good performance thanks to the efficacy of our framework, but lags behind the results when NeRF is applied to serve as a bridge between the raw Lidar data and the NOCS network.

\begin{table}
    \centering
    \renewcommand{\arraystretch}{1.1}
    \resizebox{1.0\columnwidth}{!}{%
        \input{tables/supp_withoutnerf}}
    \caption{$AP_{3D}$ from directly training with raw depth supervision from Lidar and its completion w/o NeRF.}
    \label{table:withoutnerf}
\end{table}







\noindent\textbf{Network architectures.}
We study the performance with different backbone network architectures and different NeRF configurations. Our default setup uses ResNet50 and the grid NeRF with five resolution scales as described in \cref{sec:nerf_details}.
We first change ResNet50 to ResNet18 and ResNet34, only observing slightly degraded performance. This indicates NeurOCS does not heavily rely on powerful backbone, and a lighter backbone is viable in  latency-sensitive applications.
%The runtime performance trade-off is detailed in \cref{sec:supp_runtime}. 
Next, we reduce the number of NeRF scales to 4 (finest scale with $16\!\times\!16\!\times\!16$ grids) and 3 (finest scale with $8\!\times\!8\!\times\!8$ grids), where the performance %degrades slightly.
remains good. We further substitute the grid-based NeRF to a MLP-based NeRF with positional encoding same as \cite{jang2021codenerf}. In practice, we observe the MLP-based NeRF leads to nearly two times slower training process and higher memory occupancy due to its large MLP network, while the performance drops slightly.
%its performance is similar to a 3-scale grid NeRF.
\begin{table}
    \centering
    \renewcommand{\arraystretch}{1.3}
    \resizebox{1.0\columnwidth}{!}{%
        \input{tables/supp_ablation_network_arch}
    }
    \caption{Evaluation with $AP_{3D}$ on different backbone network architectures and NeRF configurations.}
    \label{table:supp_ablation_network_arch}
\end{table}





\noindent \textbf{Scale fusion.} In the main paper, our scale fusion is described as an averaging between scales in PnP and network-predicted object depth. In fact, we have studied the generic linear combination of the two, \ie,
%We generalize the scale fusion used in main paper by adding a linear fusion weight $w$ as
\begin{equation}
\begin{gathered}
    \mathbf{s}' =  \frac{w \cdot d_{pred}+ (1-w)\cdot[\mathbf{t}]_z}{2\cdot[\mathbf{t}]_z}\,\mathbf{s}. 
    \\
    \mathbf{t}' = \frac{w \cdot d_{pred}+ (1-w)\cdot[\mathbf{t}]_z}{2\cdot[\mathbf{t}]_z}\,\mathbf{t}.
\end{gathered}
\end{equation}
%where larger $w$ indicates the scale is relying more from direct depth estimation $d_{pred}$, while lower $w$ relying more on the PnP depth $[\mathbf{t}]_z$ estimated from the object size prediction $\mathbf{s}$.
where $w$ is a balancing weight.
%The main paper defaults $w$ to 0.5. 
We study different weight values in \cref{fig:fusew}, and empirically found 0.5 (\ie averaging) gives the overall best result, which indicates similar reliability for direct depth prediction and object size prediction that gives the metric scale in PnP solutions. We have also attempted to learn the fusion using networks akin to \cite{li2022diversity}, but found this scheme to be superior in practice.
%In Fig.\ref{fig:fusew}, we study the effect of scale fusion weight.

\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{plots/ablation_fusew.pdf}
    \caption{\textbf{Effect of Fusion Weight.} Lower weight value indicates lower impact from direct depth estimation and higher impact from scale in PnP solution.}
    \label{fig:fusew}
\end{figure}




%All these time are only for 3D localization that assumes given 2D detection.

\noindent \textbf{Visual scope.}
In the main paper we have studied the behavior of object-centric and scene-centric training in NeurOCS with NeRF. Here, we study the performance when training NOCS with Lidar directly without using NeRF-rendered supervision. This allows us to focus on the image-conditioned regression branch, although we observe the NeRF branch behaves similarly in the two schemes. The results are shown in \cref{table:objectscenecentric}. In addition to the vanilla scene-centric scheme, we replace its NOCS map prediction with the one from object-centric scheme, while keeping its object mask and score prediction; this setting is denoted as ``scene-centric++". As can be seen, while a performance gap exists between the object-centric and scene-centric training, scene-centric++ largely reduces the gap especially for the Moderate and Hard cases. This demonstrates the benefits of object-centric training towards more accurate NOCS map predictions. We also increase the network capacity in the scene-centric NOCS regression head by doubling its number of layers, but do not observe consistent improvements, as shown in ``scene-centric-L". Furthermore, we evaluate scene-centric scheme with DLA as the backbone, and similar results are observed.

\begin{table}
    \centering
    \renewcommand{\arraystretch}{1.1}
    \resizebox{1.0\columnwidth}{!}{%
        \input{tables/supp_objectscenecentric}}
    \caption{Additional study on the benefits of object-centric training.}
    \label{table:objectscenecentric}
\end{table}


%\noindent \textbf{Bi-directional consistency.} The ablation study in main paper shows slight AP improvements by enforcing the bi-directional NOCS consistency (i.e. optimizing NeRF through the NOCS consistency loss). While its impact is relatively small, we observe that the bi-directional consistency may lead to slightly smoother and more structured shapes, with a few examples shown in \cref{fig:bidir}.
%We attach its qualitative result in Fig.\ref{fig:bidir}, showing slightly smoother and ordered shape at circled regions. 


\noindent \textbf{Uncertainty map.} As aforementioned, we learn a uncertain map for NOCS predictions using the reprojection loss, for both our w/ NeRF settings (NeurOCS) and those w/o NeRF baselines. We found that including the uncertainty map in the weight of PnP optimization improves the final performance. Here, we report in \cref{table:withoutuncertainty} the accuracy of NeurOCS in the case of without using it. 

\begin{table}[t]
    \centering
    \renewcommand{\arraystretch}{1.1}
    \resizebox{1.0\columnwidth}{!}{%
        \input{tables/supp_withoutuncertainty}}
    \caption{$AP_{3D}$ from NeurOCS without using the uncertainty map.}
    \label{table:withoutuncertainty}
\end{table}


\noindent \textbf{Note on NeRF.} While the shape rendering from NeRF is only required during training, we observe that it also works well for the validation set. We demonstrate this in \cref{fig:nerfshape} with an example object instance from the validation set.

\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\linewidth, trim = 0mm 122mm 50mm 0mm, clip]{figures/rebuttal_backview.pdf}
  \centering
  \caption{Shape visualization for an example object instance from the validation set.}
  \label{fig:nerfshape}  
\end{figure}


\noindent \textbf{Qualitative results.} We demonstrate the output of NeurOCS by running on KITTI raw sequences that have no overlap with the training set. In particular, the sequences are from the KITTI-Tracking subset where ground truth 3D boxes are provided for every frame. These results are shown in the attached supplementary video.



\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.1}
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{l|ccc|ccc}
\hline
                             & \multicolumn{3}{c|}{DID-M3D} & \multicolumn{3}{c}{NeurOCS-MLC} \\ \cline{2-7} 
\multirow{2}{*}{Pedestraian} & Easy    & Moderate   & Hard  & Easy     & Moderate    & Hard   \\
                             & 11.27   & 8.75       & 7.15  & 12.13    & 9.21        & 7.40   \\ \hline
\end{tabular}}
\caption{$AP_{3D}$ on the pedestrian class in KITTI validation set.}
\label{table:pedestrian}
\end{table}

\noindent \textbf{Other object classes.} We report in \cref{table:pedestrian} the results on the pedestrian class; we omit cyclists as their instance masks are not provided by~\cite{heylen2021monocinis}. As shown, NeurOCS improves upon its base detector DID-M3D despite the non-rigid object topology, further indicating its robustness.

\noindent \textbf{Computation efficiency.}\label{sec:supp_runtime}
The runtime of our framework without TTA costs 50ms on average for each frame in KITTI object dataset on a single RTX2080. The ResNet50 backbone takes about 15ms and the pose solver costs 35ms, while the TTA doubles the backbone runtime. 


\subsection{Evaluation on Waymo}
\begin{table}[t]
\centering
\vspace{-0.2cm}
\renewcommand{\arraystretch}{1.2}
\resizebox{1.0\columnwidth}{!}{
    \input{tables/waymo}}
\caption{Evaluation on Waymo dataset with $IoU{\ge}0.7$.}
\label{tab:waymo}
\vspace{-0.2cm}
\end{table}

Here, we follow~\cite{kumar2022deviant,lian2022monojsg,wang2021progressive} to train on the Waymo~\cite{Sun_2020_CVPR} dataset, only using its front camera for the monocular 3D detection task.
The Waymo dataset contains 798 training sequences and 202 validation sequences, each with around 200 images. The objects are split into two difficulty level: ``Level\_1" and ``Level\_2", depending on the number of Lidar points within the object bounding box. For evaluation, we adopt the official metrics - 3D average precision $AP_{3D}$ and 3D average precision weighted by heading $APH_{3D}$. Besides evaluating all objects together, we also evaluate for objects separately in different distance ranges, including 0-30m, 30-50m, and 50m-$\infty$. We use the panoptic annotations in Waymo to extract instance masks, which are however provided only for a subset of images - as a result we train with 12128 images instead of 52386 as in \cite{kumar2022deviant,lian2022monojsg,wang2021progressive}.  Since DID-M3D~\cite{peng2022did} does not release the code for Waymo, we instead use DEVIANT~\cite{kumar2022deviant} as our base 3D detector. As shown in \cref{tab:waymo}, despite slightly lagging behind \cite{kumar2022deviant}, our method overall outperforms other recent methods~\cite{lian2022monojsg,wang2021progressive} even without fusion. This indicates the promising potential of our method towards 3D detection in more diverse and complex environment. Empirically, we observe that the 3D object bounding box annotations in Waymo are often not tight. This may affect the learning on object size and further on the localization accuracy of NeurOCS, since the object size directly impacts the object distance in the PnP optimization. Further, the rolling shutter effect~\cite{zhuang2017rolling} in the camera used by Waymo may impact our geometric optimization which  assumes the image is taken from a global shutter camera. We leave the handling of these challenges for performance improvements as the future work. 

%We applied the same training setup as in KITTI, but envision improved performance with adaptations, \eg increasing model capacity, which are omitted due to the time constraint during rebuttal.


\subsection{Evaluation on NuScenes}

\begin{table}[t]
    \centering
    \renewcommand{\arraystretch}{1.1}
    \resizebox{1.0\columnwidth}{!}{%
        \input{tables/supp_nuscenes_deviant}
    }
    \caption{\textbf{Cross-dataset evaluation on NuScenes.} The depth MAEs are reported for recalled objects in different ranges, each containing \# objects as shown.}
    \label{table:nuscenes_deviant}
\end{table}


While cross-dataset generalization is not the main goal of our work, we follow DEVIANT~\cite{kumar2022deviant} to perform evaluation in NuScenes dataset~\cite{caesar2020nuscenes} to understand its generalization capability.  Specifically, we train on the training split of the KITTI training set and evaluate on all 6019 frontal images in the NuScenes validation set, using the mean absolute error (MAE)~\cite{kumar2022deviant,shi2021geometry} of the depth of the boxes. This is computed only on recalled objects (2D IoU$>
$0.7) where the ground truth depth can be retrieved; strictly speaking, the 3D error measured by depth MAE from two methods are comparable only when using the same set of recalled objects. We first compare with DEVIANT as shown in \cref{table:nuscenes_deviant}, where we use DEVIANT as our base detector to have the same set of recalled objects. As can be seen, while DEVIANT achieves good performance due to its special design in depth-equivariant architecture, NeurOCS yields reasonable performance with PnP alone, and its fusion with DEVIANT leads to improvements in some cases especially for nearby objects. Similar observations are obtained when using DID-M3D as the base detector. These results indicate the promising potential of NeurOCS in generalization due to its underlying geometric principles, especially for the near field where the PnP solution is less sensitive to the error in object size prediction. Further explorations towards improving its generalization capability remain our future work. 







==> tables/BACKUP_supp_objectscenecentric.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\renewcommand\arraystretch{2.0}
\begin{tabular}{cl|ccc|ccc}
\hline
\multicolumn{1}{l}{}                      & \multicolumn{1}{c|}{\multirow{2}{*}{}}                               & \multicolumn{3}{c|}{PnP Only}                                       & \multicolumn{3}{c}{+ Fusion}                                       \\ \cline{3-8} 
\multicolumn{1}{l}{}                      & \multicolumn{1}{c|}{}                                                & Easy                 & Moderate             & Hard                  & Easy                 & Moderate             & Hard                 \\ \hline
%\multicolumn{1}{c|}{\multirow{3}{*}{NeurOCS}} & object-centric &   28.46 & 18.68 & 16.22 & 31.18 & 20.90 & 17.71  \\ \cline{2-8} 
%\multicolumn{1}{c|}{}                     & \renewcommand\arraystretch{0.8}\begin{tabular}[c]{@{}c@{}}scene-centric\\ (resnet)\end{tabular} &   24.28 & 16.57 & 13.63 & 28.11  & 19.17 & 16.32 \\ \cline{2-8} 
%\multicolumn{1}{c|}{}                     &   \renewcommand\arraystretch{0.8}\begin{tabular}[c]{@{}c@{}}scene-centric\\ (dla)\end{tabular} &  23.05 & 15.42  & 12.51  & 26.87 & 18.23 & 15.00           \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{\renewcommand\arraystretch{1.6}\begin{tabular}[c]{@{}c@{}} Lidar\end{tabular}}} & object-centric &  27.15  & 18.04 & 14.91 & 30.19 & 20.32 & 17.04 \\ \cline{2-8} 
\multicolumn{1}{c|}{}                     & \renewcommand\arraystretch{0.8}\begin{tabular}[c]{@{}c@{}}scene-centric\\ (resnet)\end{tabular}  &  25.89 & 17.14 & 14.37 & 28.53 & 19.48 &  16.65 \\ \cline{2-8} 
\multicolumn{1}{c|}{}& \renewcommand\arraystretch{0.8}\begin{tabular}[c]{@{}c@{}}scene-centric-L\\ (resnet)\end{tabular}& \multicolumn{1}{l}{24.71} & \multicolumn{1}{c}{16.20} & \multicolumn{1}{l|}{13.38} & \multicolumn{1}{l}{28.00} & \multicolumn{1}{c}{18.98} & \multicolumn{1}{l}{16.13} \\ \cline{2-8} 

\multicolumn{1}{c|}{}& \renewcommand\arraystretch{0.8}\begin{tabular}[c]{@{}c@{}}scene-centric++\\ (resnet)\end{tabular}& \multicolumn{1}{c}{26.53} & \multicolumn{1}{c}{17.91} & \multicolumn{1}{l|}{14.82} & \multicolumn{1}{l}{29.16} & \multicolumn{1}{c}{20.15} & \multicolumn{1}{l}{16.87} \\ \cline{2-8} 

\multicolumn{1}{c|}{}&\renewcommand\arraystretch{0.8}\begin{tabular}[c]{@{}c@{}}scene-centric\\ (dla)\end{tabular} &24.38 & 16.07  & 13.13 & 27.49 & 18.55 & 15.31  \\ \cline{2-8}

\multicolumn{1}{c|}{}&\renewcommand\arraystretch{0.8}\begin{tabular}[c]{@{}c@{}}scene-centric++\\ (dla)\end{tabular} & 26.23  & 17.82  & 14.82 & 29.05 & 20.12  & 16.97   \\ \hline


\multicolumn{1}{c|}{\multirow{5}{*}{\renewcommand\arraystretch{2.0}\begin{tabular}[c]{@{}c@{}}  \renewcommand\arraystretch{0.8}\begin{tabular}[c]{@{}c@{}}Lidar+\\ Lidar Comp.\end{tabular} \end{tabular}}} & object-centric & 28.01 & 18.39 & 15.63 & 30.42 & 20.58 & 17.23 \\ \cline{2-8} 

\multicolumn{1}{l|}{}&\renewcommand\arraystretch{0.8}\begin{tabular}[c]{@{}c@{}}scene-centric\\ (resnet)\end{tabular} &  26.23 & 16.76 & 14.05 & 28.33 & 19.12 & 16.03 \\ \cline{2-8} 

\multicolumn{1}{l|}{}&\renewcommand\arraystretch{0.8}\begin{tabular}[c]{@{}c@{}}scene-centric++\\ (resnet)\end{tabular} &  27.18 & 18.49 & 15.56  & 29.45 & 20.31 & 17.12 \\ \cline{2-8} 

\multicolumn{1}{l|}{}& \renewcommand\arraystretch{0.8}\begin{tabular}[c]{@{}c@{}}scene-centric\\ (dla)\end{tabular}& 24.16 &  16.01 & 13.03 & 28.08 &18.69 & 15.45 \\ \cline{2-8} 

\multicolumn{1}{l|}{}& \renewcommand\arraystretch{0.8}\begin{tabular}[c]{@{}c@{}}scene-centric++\\ (dla)\end{tabular}& 26.94  & 18.41  & 15.28  & 29.42 & 20.31 & 17.13 \\ \hline

\end{tabular}


==> tables/bbback_benchmark.tex <==
\begin{tabular}{ccccccccccccccc}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{Method}} &
\multicolumn{1}{c|}{\multirow{2}{*}{Venue}} &
\multicolumn{1}{c|}{\multirow{2}{*}{Cat.}} &
\multicolumn{3}{c|}{3D $AP_{40} $ - Test} & \multicolumn{3}{c||}{3D $AP_{40} $ - Val} & \multicolumn{3}{c|}{BEV $AP_{40} $ - Test}  & \multicolumn{3}{c}{BEV $AP_{40} $ - Val} \\

%\cline{3-14} 
\cline{4-15} 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &
\multicolumn{1}{c|}{} & Easy & Moderate & \multicolumn{1}{c|}{Hard} & Easy & Moderate & \multicolumn{1}{c||}{Hard} & Easy & Moderate & \multicolumn{1}{c|}{Hard} & Easy & Moderate & Hard \\ \hline

\multicolumn{1}{c|}{Monodle~\cite{ma2021delving}} & 
\multicolumn{1}{c|}{CVPR21} &
\multicolumn{1}{c|}{E} &
17.23 & 12.26 & \multicolumn{1}{c|}{10.29}  &
17.45 & 13.66 & \multicolumn{1}{c||}{11.68} &
24.79 & 18.89 & \multicolumn{1}{c|}{16.00}  &
24.97 & 19.33 & 17.01 \\

 \multicolumn{1}{c|}{MonoEF~\cite{zhou2021monocular}} & 
 \multicolumn{1}{c|}{CVPR21} &
 \multicolumn{1}{c|}{E} &
 21.29& 13.87 & \multicolumn{1}{c|}{11.71}  &
 -&  -& \multicolumn{1}{c||}{-} &
 29.03& 19.70 & \multicolumn{1}{c|}{17.26}  &
 -&  -& - \\
 
  \multicolumn{1}{c|}{DDMP-3D~\cite{wang2021depth}} & \multicolumn{1}{c|}{CVPR21} &
\multicolumn{1}{c|}{E} &
 19.71 & 12.78 & \multicolumn{1}{c|}{9.80}  &
 \textcolor{MidnightBlue}{28.12} & \textcolor{MidnightBlue}{20.39} & \multicolumn{1}{c||}{\textcolor{MidnightBlue}{16.34}} &
 28.08 & 17.89 & \multicolumn{1}{c|}{13.44}  &
 -& - & -  \\ 

 \multicolumn{1}{c|}{CaDDN~\cite{reading2021categorical}} & \multicolumn{1}{c|}{CVPR21} &
\multicolumn{1}{c|}{E} &
 19.17& 13.41 & \multicolumn{1}{c|}{11.46}  &
 23.57& 16.31 & \multicolumn{1}{c||}{13.84} &
 27.94 & 18.91  &  \multicolumn{1}{c|}{17.19}  &
 -& - & - \\ 
 
 
  \multicolumn{1}{c|}{GrooMeD-NMS~\cite{kumar2021groomed}} & \multicolumn{1}{c|}{CVPR21} &
\multicolumn{1}{c|}{E} &
 18.10 & 12.32  & \multicolumn{1}{c|}{9.65}  &
 19.67 & 14.10 & \multicolumn{1}{c||}{10.47} &
 26.19 & 18.27  & \multicolumn{1}{c|}{14.05}  &
 27.38 & 19.75  & 15.92 \\ 
 
 %\multicolumn{1}{c|}{DD3D~\cite{park2021pseudo}} & \multicolumn{1}{c|}{ICCV21} &
%\multicolumn{1}{c|}{E} &
% 23.19 & 16.87 & \multicolumn{1}{c|}{14.36}  &
% 32.35 & 23.41 & \multicolumn{1}{c||}{20.42}  &
% &  & \multicolumn{1}{c|}{} &
% &  &  \\ 


\multicolumn{1}{c|}{PCT~\cite{wang2021progressive}} &
\multicolumn{1}{c|}{NeurIPS21} &
\multicolumn{1}{c|}{E} &
21.00 & 13.37 & \multicolumn{1}{c|}{11.31}  &
\textcolor{MidnightBlue}{38.39} & \textcolor{MidnightBlue}{27.12} & \multicolumn{1}{c||}{\textcolor{MidnightBlue}{24.11}} &
29.65 & 19.03 & \multicolumn{1}{c|}{15.92}  &
\textcolor{MidnightBlue}{47.16} & \textcolor{MidnightBlue}{34.65} & \textcolor{MidnightBlue}{28.47} \\ 

\multicolumn{1}{c|}{MonoGround~\cite{qin2022monoground}} & \multicolumn{1}{c|}{CVPR22} &
\multicolumn{1}{c|}{E} &
 21.37 & 14.36 & \multicolumn{1}{c|}{12.62}  &
 25.24 & 18.69 & \multicolumn{1}{c||}{15.58} &
 30.07& 20.47 & \multicolumn{1}{c|}{17.74}  &
 32.68& 24.79 & 20.56  \\ 

\multicolumn{1}{c|}{HomoLoss~\cite{gu2022homography}} & \multicolumn{1}{c|}{CVPR22} &
\multicolumn{1}{c|}{E} &
 21.75 & 14.94 & \multicolumn{1}{c|}{13.07}  &
 23.04 & 16.89  & \multicolumn{1}{c||}{14.90} &
 29.60& 20.68 & \multicolumn{1}{c|}{17.81}  &
 31.04& 22.99 & 19.84 \\ 
 
 
\multicolumn{1}{c|}{MonoDTR~\cite{huang2022monodtr}} & \multicolumn{1}{c|}{CVPR22} &
\multicolumn{1}{c|}{E} &
 21.99 & 15.39 & \multicolumn{1}{c|}{12.73}  &
 24.52 & 18.57  & \multicolumn{1}{c||}{15.51} &
 28.59 & 20.38 & \multicolumn{1}{c|}{17.14}  &
 33.33 & 25.35 & 21.68 \\ 

\multicolumn{1}{c|}{PseudoStereo~\cite{chen2022pseudo}} & \multicolumn{1}{c|}{CVPR22} &
\multicolumn{1}{c|}{E} &
 23.74& 17.74  & \multicolumn{1}{c|}{15.14}  &
 \textcolor{MidnightBlue}{35.18} & \textcolor{MidnightBlue}{24.15} & \multicolumn{1}{c||}{\textcolor{MidnightBlue}{20.35}} &
 32.84 & 23.67  & \multicolumn{1}{c|}{20.64}  &
 -& -  & - \\ 
 

\multicolumn{1}{c|}{DEVIANT~\cite{kumar2022deviant}} & \multicolumn{1}{c|}{ECCV22} &
\multicolumn{1}{c|}{E} &
 21.88 & 14.46 & \multicolumn{1}{c|}{11.89}  &
 24.63 & 16.54 & \multicolumn{1}{c||}{14.52} &
 29.65 & 20.44 & \multicolumn{1}{c|}{17.43}  &
 32.60 & 23.04 & 19.99 \\ 


\multicolumn{1}{c|}{DID-M3D~\cite{peng2022did}} & \multicolumn{1}{c|}{ECCV22} &
\multicolumn{1}{c|}{E} &
24.40 & 16.29 & \multicolumn{1}{c|}{13.75}  &
22.98 & 16.12 & \multicolumn{1}{c||}{14.03} &
32.95 & 22.76 & \multicolumn{1}{c|}{19.83}  &
31.10 & 22.76 & 19.50 \\ \hline\hline

%\multicolumn{1}{c|}{MoGDE~\cite{mogde2022}} &
%\multicolumn{1}{c|}{NeurIPS22} &
%\multicolumn{1}{c|}{E} &
% &  & \multicolumn{1}{c|}{}  &
% &  & \multicolumn{1}{c||}{} &
% &  & \multicolumn{1}{c|}{}  &
%- & - & - \\ 

\multicolumn{1}{c|}{MonoRUn~\cite{chen2021monorun}} &
\multicolumn{1}{c|}{CVPR21} &
\multicolumn{1}{c|}{H} &
19.65 & 12.30 & \multicolumn{1}{c|}{10.58}  &
20.02 & 14.65 & \multicolumn{1}{c||}{12.61} &
27.94 & 17.34 & \multicolumn{1}{c|}{15.24}  &
- & - & - \\

%\multicolumn{1}{c|}{*EProPnP} & \multicolumn{1}{c|}{P} & - & - & \multicolumn{1}{c|}{-} &  &  & \multicolumn{1}{c||}{} & - & - & \multicolumn{1}{c|}{-} &  &  &  \\

\multicolumn{1}{c|}{MonoRCNN~\cite{shi2021geometry}} & % 
\multicolumn{1}{c|}{ICCV21} &
\multicolumn{1}{c|}{E} &
18.36 & 12.65 & \multicolumn{1}{c|}{10.03}  &
16.61 & 13.19 & \multicolumn{1}{c||}{10.65} &
25.48 & 18.11 & \multicolumn{1}{c|}{14.10}  &
25.29 & 19.22 & 15.30 \\ 

\multicolumn{1}{c|}{GUPNet~\cite{lu2021geometry}} &
\multicolumn{1}{c|}{ICCV21} &
\multicolumn{1}{c|}{H} &
22.26 & 15.02  &  \multicolumn{1}{c|}{13.12} &
22.76 & 14.46  & \multicolumn{1}{c||}{13.72} &
30.29 & 21.19  &  \multicolumn{1}{c|}{18.20} &  
31.07 & 22.94  & 19.75\\
      
\multicolumn{1}{c|}{Autoshape~\cite{liu2021autoshape}} &
\multicolumn{1}{c|}{ICCV21} &
\multicolumn{1}{c|}{P} &
22.47 & 14.17 & \multicolumn{1}{c|}{11.36}  & 
20.09 & 14.65 & \multicolumn{1}{c||}{12.07} &
30.66 & 20.08 & \multicolumn{1}{c|}{15.95}  &
- & - & - \\

\multicolumn{1}{c|}{DCD~\cite{li2022densely}} &
\multicolumn{1}{c|}{ECCV22} &
\multicolumn{1}{c|}{K} &
23.81 & 15.90 & \multicolumn{1}{c|}{13.21}  &
23.94 & 17.38 & \multicolumn{1}{c||}{15.32} &
32.55 & 21.50 & \multicolumn{1}{c|}{18.25}  &
- & - & - \\

%\multicolumn{1}{c|}{Ours} & \multicolumn{1}{c|}{P} & \textbf{25.68} & \textbf{16.52} & \multicolumn{1}{c|}{\textbf{13.85}} & \textbf{29.78} & \textbf{19.19} & \multicolumn{1}{c||}{\textbf{16.59}} & \textbf{32.82} & \textbf{21.69} & \multicolumn{1}{c|}{\textbf{18.53}} & \textbf{36.78} & \textbf{25.08} & \textbf{21.37} \\ \hline % best val model
\multicolumn{1}{c|}{\textbf{Ours-PnP}} &
\multicolumn{1}{c|}{-} &
\multicolumn{1}{c|}{P} &
\textbf{25.68} & \textbf{16.52} & \multicolumn{1}{c|}{\textbf{13.85}}  &
\textbf{28.46} & \textbf{18.68} & \multicolumn{1}{c||}{\textbf{16.22}} &
\textbf{32.82} & \textbf{21.69} & \multicolumn{1}{c|}{\textbf{18.53}}  &
\textbf{35.65} & \textbf{24.55} & \textbf{20.98} \\ \hline\hline % avg val model

\multicolumn{1}{c|}{MonoFlex~\cite{zhang2021objects}} &
\multicolumn{1}{c|}{CVPR21} &
\multicolumn{1}{c|}{EH} &
19.94 & 13.89 & \multicolumn{1}{c|}{12.07}  &
23.64 & 17.51 & \multicolumn{1}{c||}{14.83} &
28.23 & 19.75 & \multicolumn{1}{c|}{16.89}  &
- & - & - \\

\multicolumn{1}{c|}{MonoJSG~\cite{liu2021autoshape}} &
\multicolumn{1}{c|}{CVPR22} &
\multicolumn{1}{c|}{EP} &
24.69& 16.14 & \multicolumn{1}{c|}{13.64}  & 
26.4 & 18.3 & \multicolumn{1}{c||}{15.4} &
32.59 & 21.26 & \multicolumn{1}{c|}{18.18}  &
- & - & - \\

\multicolumn{1}{c|}{MonoDDE~\cite{li2022diversity}} &
\multicolumn{1}{c|}{CVPR22} &
\multicolumn{1}{c|}{EHK} &
24.93 & 17.14 & \multicolumn{1}{c|}{15.10}  &
26.66 & 19.75 & \multicolumn{1}{c||}{16.72} &
33.58 & 23.46 & \multicolumn{1}{c|}{20.37}  &
35.51 & 26.48 & 23.07 \\

%\multicolumn{1}{c|}{Ours +\cite{peng2022did}} & \multicolumn{1}{c|}{PE} & \textbf{28.68} & \textbf{18.46} & \multicolumn{1}{c|}{\textbf{15.63}} & \textbf{32.07} & \textbf{21.35} & \multicolumn{1}{c||}{\textbf{18.54}} & \textbf{37.38} & \textbf{24.41} & \multicolumn{1}{c|}{\textbf{20.95}} & \textbf{40.15} & \textbf{27.78} & \textbf{23.88} \\ \hline % best val model
\multicolumn{1}{c|}{\textbf{Ours-Fusion}} &
\multicolumn{1}{c|}{-} &
\multicolumn{1}{c|}{EP} &
\textbf{28.68} & \textbf{18.46} & \multicolumn{1}{c|}{\textbf{15.63}} &
\textbf{31.18} & \textbf{20.90} & \multicolumn{1}{c||}{\textbf{17.71}}&
\textbf{37.38} & \textbf{24.41} & \multicolumn{1}{c|}{\textbf{20.95}} &
\textbf{39.54} & \textbf{27.25} & \textbf{23.64} \\ \hline % avg val model
\multicolumn{15}{r}{\small{\textbf{P} = PnP (and its variants), \; \textbf{E} = Direct depth estimation, \; \textbf{H} = Depth from height, \; \textbf{K} = Depth from keypoints}}
\end{tabular}

==> tables/supp_ablation_network_arch.tex <==
\begin{tabular}{c|c|ccc|ccc}
\hline
\multirow{2}{*}{Module} & \multirow{2}{*}{Model} & \multicolumn{3}{c|}{PnP Only} & \multicolumn{3}{c}{+ Fusion} \\ \cline{3-8} 
 &  & Easy & Moderate & Hard & Easy & Moderate & Hard \\ \hline
 \multirow{1}{*}{Default} & ResNet50+5 Grid Scales & 27.92 & 18.49 & 15.78 & 31.24 &21.01 & 17.70 \\ \hline
 \multirow{2}{*}{Backbone} & ResNet18 & 27.04 & 18.21 & 15.39 & 30.18 & 20.80 & 17.44 \\
 & ResNet34 & 27.00 & 18.19 & 15.47 & 30.39 & 20.71 & 17.38\\ \hline
\multirow{3}{*}{NeRF} & 4 Grid Scales & 27.80 & 18.49 & 15.81 & 30.93 & 20.90 & 17.56\\
 & 3 Grid Scales & 28.02 & 18.62 & 15.89 & 31.16 & 21.02 & 17.64\\
 & CodeNeRF & 27.41 & 18.23 & 15.10 & 30.53 & 20.77 & 17.45  \\ \hline
\end{tabular}

==> tables/supp_comparewith_cmkd.tex <==
\begin{tabular}{l|c|lll|lll}
\multirow{2}{*}{Method} & \multirow{2}{*}{Venue} & \multicolumn{3}{c|}{3D $AP_{40} $ - Test} & \multicolumn{3}{c}{BEV $AP_{40} $ - Test} \\ \cline{3-8} 
                        &                        & Easy       & Mod      & Hard      & Easy      & Mod      & Hard      \\ \hline
                      LPCG~\cite{peng2022lidar}  & ECCV22 & 25.56 & 17.80 & 15.38 & 35.96 & 24.81 & 21.86  \\
                      CMKD~\cite{hong2022cross} & ECCV22 & 28.55 & 18.69 & 16.77 & 38.98 & 25.82 & 22.80 \\
                      NeurOCS  & CVPR23 &  29.89 & 18.94 & 15.90 & 37.27 & 24.49 & 20.89
\end{tabular}



==> tables/supp_comparewith_deviant.tex <==
\begin{tabular}{c|c|lll|lll}
\multirow{2}{*}{Method} & \multirow{2}{*}{Venue} & \multicolumn{3}{c|}{3D $AP_{40} $ - Val} & \multicolumn{3}{c}{BEV $AP_{40} $ - Val} \\ \cline{3-8} 
                        &                        & Easy       & Mod      &Hard      & Easy      & Mod      & Hard      \\ \hline
DEVIANT~\cite{kumar2022deviant}  & ECCV22 &  25.09 & 16.99 & 15.30 & 33.69 & 23.10 & 20.67           \\\hline
%NeurOCS-M   & - & 22.71 & 15.78 & 14.01 & 29.32 & 21.40 &  18.79 \\
%NeurOCS-MLC  & - & 21.98& 15.73 & 13.79 & 29.33 & 21.22 & 18.64 %\\\hline    
NeurOCS-M + \cite{kumar2022deviant}  & CVPR23 & 27.70 & 18.92 & 16.28 & 35.31 & 25.11 & 21.87 \\        
NeurOCS-MLC + \cite{kumar2022deviant}  & CVPR23 & 27.83 & 18.92 & 16.20 & 35.14 & 24.77 & 21.43 \\        
\end{tabular}



==> tables/supp_losses.tex <==
\begin{tabular}{c|c|c|c|c|c}
\hline
Module & Loss Name & Type & Weight & Region & Note \\ \hline
\multirow{6}{*}{NeRF} & Occupancy Loss & L2 & 1 & FG + BG &  \\
 & RGB Loss & L2 & 3 & FG &  \\
 & KL Divergence & KL & 1 & - &  \\
 & Lidar Loss & L2 & 0.5 & FG \& Valid & Optional \\
 & LiComp Loss & L2 & 0.2 & FG \& Valid & Optional \\
 & Dense Prior & L1 & 0.002 & 3D Grid & Conditional \\ \hline
\multirow{3}{*}{Image} & FG Loss & L2 & 1 & All &  \\
 & IoU Score Loss & L2 & 1 & - &  \\
 & Reproj. Loss & L2 & 2 & FG &  \\ \hline
Both & NOCS Consistency & L2 & 1 & FG \& Occ &  \\ \hline

\multicolumn{6}{r}{\small {FG = Foreground, \; BG = Backgroud}}

\end{tabular}

==> tables/supp_nuscenes_deviant.tex <==

\begin{tabular}{c|ccc|ccc}
 & \multicolumn{3}{c|}{Mean Depth MAE}& \multicolumn{3}{c}{Median Depth MAE}\\ \hline
\begin{tabular}[c]{@{}c@{}}range\\ (\# of obj.)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0-20m\\ (596)\end{tabular} & \begin{tabular}[c]{@{}c@{}}20-40m\\ (719)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textgreater{}40m\\ (16)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0-20m\\ (596)\end{tabular} & \begin{tabular}[c]{@{}c@{}}20-40m\\ (719)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textgreater{}40m\\ (16)\end{tabular} \\ \hline
DEVIANT~\cite{kumar2022deviant}   & 0.757  & \textbf{1.603}    & \textbf{4.499}   & 0.660  & 1.270  & \textbf{4.590}  \\ 
NeurOCS-PnP  & 0.746  & 2.160    & 6.719   & 0.575  & 1.780  & 6.725  \\ 
NeurOCS-Fusion & \textbf{0.602}   & 1.714    & 5.624   & \textbf{0.460}  & \textbf{1.180}  & 5.415 \\ \hline \hline

\begin{tabular}[c]{@{}c@{}}range\\ (\# of obj.)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0-20m\\ (1273)\end{tabular} & \begin{tabular}[c]{@{}c@{}}20-40m\\ (2173)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textgreater{}40m\\ (858)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0-20m\\ (1273)\end{tabular} & \begin{tabular}[c]{@{}c@{}}20-40m\\ (2173)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textgreater{}40m\\ (858)\end{tabular} \\ \hline
DID-M3D~\cite{peng2022did}   & 0.665  & \textbf{1.713}    & \textbf{3.373}   & 0.510  & 1.400  & \textbf{2.740}  \\ 
NeurOCS-PnP   & 0.801  & 2.396    & 5.671   & 0.650  & 1.950  & 5.275  \\ 
NeurOCS-Fusion   & \textbf{0.637}  & 1.721    & 3.711   & \textbf{0.480} & \textbf{1.380}  & 3.150  \\ 

\end{tabular}


==> tables/supp_objectscenecentric.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\renewcommand\arraystretch{1.1}
\begin{tabular}{c|ccc|ccc}
\hline
 \multicolumn{1}{c|}{\multirow{2}{*}{}}                               & \multicolumn{3}{c|}{PnP Only}                                       & \multicolumn{3}{c}{+ Fusion}                                       \\ 
 \multicolumn{1}{c|}{}                                                & Easy                 & Moderate             & Hard                  & Easy                 & Moderate             & Hard                 \\ \hline
%\multicolumn{1}{c|}{\multirow{3}{*}{NeurOCS}} & object-centric &   28.46 & 18.68 & 16.22 & 31.18 & 20.90 & 17.71  \\ \cline{2-8} 
%\multicolumn{1}{c|}{}                     & \renewcommand\arraystretch{0.8}\begin{tabular}[c]{@{}c@{}}scene-centric\\ (resnet)\end{tabular} &   24.28 & 16.57 & 13.63 & 28.11  & 19.17 & 16.32 \\ \cline{2-8} 
%\multicolumn{1}{c|}{}                     &   \renewcommand\arraystretch{0.8}\begin{tabular}[c]{@{}c@{}}scene-centric\\ (dla)\end{tabular} &  23.05 & 15.42  & 12.51  & 26.87 & 18.23 & 15.00           \\ \hline
 object-centric &  27.92 & 18.49 & 15.78 & 31.24 &21.01 & 17.70 \\ \hline 
 \renewcommand\arraystretch{0.8}\begin{tabular}[c]{@{}c@{}}scene-centric\\ (resnet)\end{tabular}  &  26.39 &17.62 & 14.61 & 29.40 & 20.20 & 16.94 \\ \hline 
 
\renewcommand\arraystretch{0.8}\begin{tabular}[c]{@{}c@{}}scene-centric++\\ (resnet)\end{tabular}& 25.30 & 18.02 & 15.64 & 28.54 & 20.60 & 17.57 \\ \hline 

\renewcommand\arraystretch{0.8}\begin{tabular}[c]{@{}c@{}}scene-centric-L\\ (resnet)\end{tabular}& 25.95 & 17.35 & 14.51 & 29.57 & 20.39 & 17.06  \\ \hline  

\renewcommand\arraystretch{0.8}\begin{tabular}[c]{@{}c@{}}scene-centric\\ (dla)\end{tabular} & 25.04 & 16.89 & 14.03 & 28.48 & 19.34 & 16.26\\ \hline 

\renewcommand\arraystretch{0.8}\begin{tabular}[c]{@{}c@{}}scene-centric++\\ (dla)\end{tabular} & 26.00 & 18.05 & 15.81 & 29.25 & 20.60 & 17.55   \\ \hline

\end{tabular}


==> tables/supp_withoutnerf.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\renewcommand\arraystretch{1.1}
\begin{tabular}{l|ccc|ccc}
\hline
 \multicolumn{1}{c|}{\multirow{2}{*}{}}                               & \multicolumn{3}{c|}{PnP Only}                                       & \multicolumn{3}{c}{+ Fusion}                                       \\ 
 \multicolumn{1}{c|}{}                                                & Easy                 & Moderate             & Hard                  & Easy                 & Moderate             & Hard                 \\ \hline
 RLC & 27.55 & 18.27 & 15.75 & 30.79 & 20.78 & 17.37   \\ 
 RL &  27.50 & 18.36 & 15.77 & 30.45 & 20.71 & 17.45 \\ 
 RC &  27.08 & 18.10 & 15.28 & 30.74 & 20.67 & 17.41 \\ 
 R &   22.59 & 15.81 & 13.07 & 27.26 & 19.10 & 16.48\\
 \hline
\end{tabular}


==> tables/supp_withoutuncertainty.tex <==
\renewcommand\arraystretch{1.1}
\begin{tabular}{l|ccc|ccc}
\hline
 \multicolumn{1}{c|}{\multirow{2}{*}{}}                               & \multicolumn{3}{c|}{PnP only}                                       & \multicolumn{3}{c}{+ Fusion}                                       \\ 
 \multicolumn{1}{c|}{}                                                & Easy                 & Moderate             & Hard                  & Easy                 & Moderate             & Hard                 \\ \hline
 NeurOCS-MLC &  28.06 & 18.52 & 15.36 & 31.20 & 20.99 & 17.55\\ 
 NeurOCS-ML  &  28.23 & 18.58 & 15.49 & 30.79 & 20.80 & 17.48\\ 
 NeurOCS-MC  &  28.07 & 18.69 & 15.82 & 30.93 & 20.87 & 17.46\\ 
 NeurOCS-M   &  27.66 & 18.42 & 15.54 & 30.66 & 20.77 & 17.49\\
 \hline
\end{tabular}


==> tables/waymo.tex <==


\begin{tabular}{c|c|cccc|cccc}
\hline
\multirow{2}{*}{Difficulty} & \multirow{2}{*}{Method} & \multicolumn{4}{c|}{$AP_{3D}$}                          & \multicolumn{4}{c}{$APH_{3D}$}                           \\ \cline{3-10} 
                            &                         & \multicolumn{1}{c|}{All}  & 0-30m & 30-50m & 50m-$\infty$ & \multicolumn{1}{c|}{All}  & 0-30m & 30-50m & 50m-$\infty$ \\ \hline
\multirow{5}{*}{Level\_1}     & PCT~\cite{wang2021progressive}                     & \multicolumn{1}{c|}{0.89} & 3.18  & 0.27   & 0.07 & \multicolumn{1}{c|}{0.88} & 3.15  & 0.27   & 0.07 \\
                            & MonoJSG~\cite{lian2022monojsg}                 & \multicolumn{1}{c|}{0.97} & 4.65  & 0.55   & 0.10 & \multicolumn{1}{c|}{0.95} & 4.59  & 0.53   & 0.09 \\
                            & DEVIANT~\cite{kumar2022deviant}                 & \multicolumn{1}{c|}{2.69} & 6.95  & 0.99   & 0.02 & \multicolumn{1}{c|}{2.67} & 6.90  & 0.98   & 0.02 \\ \cline{2-10} 
                            & NeurOCS (PnP)           & \multicolumn{1}{c|}{1.67} & 4.28  & 0.74   & 0.02 & \multicolumn{1}{c|}{1.66} & 4.26  & 0.73   & 0.02 \\
                            & NeurOCS (Fusion)        & \multicolumn{1}{c|}{2.44} & 6.35  & 0.97   & 0.04 & \multicolumn{1}{c|}{2.43} & 6.31  & 0.97   & 0.04 \\ \hline
\multirow{5}{*}{Level\_2}     & PCT~\cite{wang2021progressive}                     & \multicolumn{1}{c|}{0.66} & 3.18  & 0.27   & 0.07 & \multicolumn{1}{c|}{0.66} & 3.15  & 0.26   & 0.07 \\
                            & MonoJSG~\cite{lian2022monojsg}                 & \multicolumn{1}{c|}{0.91} & 4.64  & 0.55   & 0.09 & \multicolumn{1}{c|}{0.89} & 4.65  & 0.53   & 0.09 \\
                            & DEVIANT~\cite{kumar2022deviant}                 & \multicolumn{1}{c|}{2.52} & 6.93  & 0.95   & 0.02 & \multicolumn{1}{c|}{2.50} & 6.87  & 0.94   & 0.02 \\ \cline{2-10} 
                            & NeurOCS (PnP)           & \multicolumn{1}{c|}{1.56} & 4.26  & 0.71   & 0.02 & \multicolumn{1}{c|}{1.55} & 4.24  & 0.70   & 0.02 \\
                            & NeurOCS (Fusion)        & \multicolumn{1}{c|}{2.29} & 6.32  & 0.94   & 0.03 & \multicolumn{1}{c|}{2.28} & 6.29  & 0.93   & 0.03 \\ \hline
\end{tabular}

